Pre-deployment Analysis of Smart Contracts -- A Survey

Smart contracts are programs that execute transactions involving independent parties and cryptocurrencies. As programs, smart contracts are susceptible to a wide range of errors and vulnerabilities. Such vulnerabilities can result in significant losses. Furthermore, by design, smart contract transactions are irreversible. This creates a need for methods to ensure the correctness and security of contracts pre-deployment. Recently there has been substantial research into such methods. The sheer volume of this research makes articulating state-of-the-art a substantial undertaking. To address this challenge, we present a systematic review of the literature. A key feature of our presentation is to factor out the relationship between vulnerabilities and methods through properties. Specifically, we enumerate and classify smart contract vulnerabilities and methods by the properties they address. The methods considered include static analysis as well as dynamic analysis methods and machine learning algorithms that analyze smart contracts before deployment. Several patterns about the strengths of different methods emerge through this classification process.

==> BackUP/AllTables.tex <==
%%------------ Table of Properties vs vulnerabilities ------------%%
\begin{table*}
 \vspace{-2mm}
\setlength\abovecaptionskip{-0.1\baselineskip}
  \setlength\belowcaptionskip{-0.1\baselineskip}
  \caption{Smart contract properties with related vulnerabilities and studies. Liveness properties are represented with$^\ast$}
  \label{tab:propVuln}
   \resizebox{\columnwidth}{90mm}{
  \begin{tabular}{| p{40mm} | p{46mm} | p{12mm} | p {60mm} |}
    \hline
    Property & Vulnerabilities & Platform & Studies \\
    \hline
    
    \multirow{2}{45mm}{Address integrity}
        & Forged notification, Fake receipt & EOSIO & \cite{huang2020eosfuzzer, he2021eosafe, li2022eosioanalyzer,Wasai2022} \\
        \cline{2-4}
        & External contract referencing & Ethereum & \cite{nelaturu2020verified} \\
    \hline
    
    Address parameter avoidance 
        & Misuse of address parameters  & Ethereum & \cite{praitheeshan2021solguard}\\
        
    \hline
    Address size soundness 
        & Address shortening & Ethereum & \cite{nelaturu2020verified, ashouri2020etherolic, xing2020new}\\
           
    \hline
           
    \multirow{2}{45mm}{Appropriate address usage}
        & Misuse of \texttt{msg.sender} &   & \cite{zhdarkin2021development}\\
        & Misuse of \texttt{tx.origin}  & Ethereum &  \cite{lu2021neucheck, arganaraz2020detection, kalra2018zeus, tikhomirov2018smartcheck, brent2018vandal}\\
        & Prodigal contract & & \cite{praitheeshan2019security, tang2021vulnerabilities}\\
        
    \hline
    
    \multirow{2}{45mm}{Asset value \& transaction preservation}
        & Unfair payment & Ethereum &\cite{li2020protect} \\ 
        \cline{2-4}
        &  Double-spending  & Algorand &\cite{bartoletti2021formal}\\
          
    \hline
    
    Balance comparison 
        & Strict equality of balance &  Ethereum & \cite{lu2021neucheck, arganaraz2020detection,tikhomirov2018smartcheck} \\
    
    \hline
           
    \multirow{3}{45mm}{Boundedness of loops}    
        & Un-bounded mass operations & Ethereum &  \cite{grech2020madmax, lu2021neucheck, nassirzadeh2021gas, Correas2021static}\\
        & Unsafe type declaration, Unsecure inference &  & \cite{lu2021neucheck, arganaraz2020detection, tikhomirov2018smartcheck} \\
      \hline
      
    Eventual termination of expressions in conditions$^\ast$  
        & DoS due to external contracts & Ethereum & \cite{arganaraz2020detection, lu2021neucheck}\\
           
    \hline
           
    \texttt{delegatecall} preservation 
        & Tainted \texttt{delegatecall} & Ethereum & \cite{brent2020ethainter, wei2020smart, teng2021SmartGift, andesta2020testing, jiang2018contractfuzzer} \\
         
    \hline
    
    \multirow{2}{45mm}{Eventual contract termination$^\ast$ } 
        & Non-terminating contracts & Ethereum & \cite{genet2020termination}  \\
        \cline{3-4}
        &   & Cardano & \cite{seijas2020efficient,Seijas2020Marlowe} \\
     
    \hline
    
    Deposit acceptance$^\ast$ 
        &  Failing to accept new deposit & Ethereum & \cite{park2020end} \\
        
    \hline
    
    \multirow{2}{45mm}{Deposit validity}
        & Fake deposit & Ethereum & \cite{ji2020deposafe} \\
        \cline{2-4}
        & Fake EOS & EOSIO & \cite{he2020security, huang2020eosfuzzer, he2021eosafe, li2022eosioanalyzer, Wasai2022} \\
        \cline{2-4}
        & Negative deposit & Cardano &  \cite{seijas2020efficient}\\
       
    \hline 
    
    Divide by zero guarding 
        & Unchecked division by zero & Ethereum & \cite{so2020verismart, Khor2020improved, Osiris2018}\\
    
    \hline
    
    Effective callback freeness & Reentrancy & Ethereum
        &\cite{albert2020taming, grossman2017online}\\   
    
    \hline
    
    \multirow{3}{40mm}{Exceptions \& return value handling}   
        & Callstack depth attack vulnerability &   & \cite{wang2020contractward}\\
        & Gasless send &  Ethereum & \cite{nguyen2020sfuzz, teng2021SmartGift, jiang2018contractfuzzer} \\
        & Mishandled/unhandled exceptions &  & \cite{zhang2020smartshield, nelaturu2020verified, ashouri2020etherolic, arganaraz2020detection, semantics2020Jiao, nguyen2020sfuzz, wei2020smart, Oyente2016, kalra2018zeus, tikhomirov2018smartcheck, grishchenko2018semantic}\\ 
    
    \hline
    
    \multirow{3}{40mm}{Explicit access control modifiers usage}
        & Tainted owner variable, Vulnerable access control & & \cite{lu2021neucheck} \\
        & Unspecified visibility level &  &  \cite{lu2021neucheck, tikhomirov2018smartcheck} \\
    
    \hline
    
    Hash collision freeness 
        & Hash collision &  Ethereum & \cite{lu2021neucheck}\\
    
    \hline
    
    Information secrecy 
        &  Exposed secret & Ethereum & \cite{zhang2020ethploit, lu2021neucheck}\\
    
    \hline 
    
    Integer over/underflow guarding 
        &  Integer over/underflow  & Ethereum 
        & \cite{ma2021pluto, ashouri2020etherolic, sun2020formal, so2020verismart, lai2020static, xing2020new, semantics2020Jiao, nguyen2020sfuzz, Khor2020improved, wang2020contractward, lu2021neucheck, yang2020hybrid, andesta2020testing,stephens2021smartpulse, kalra2018zeus,mossberg2019manticore} \\
        \cline{3-4}
        &  & HFabric & \cite{ding2021hfcontractfuzzer}\\
    
    \hline
    
    \multirow{2}{45mm}{Isolation of external calls}
        & DoS due to external contracts & Ethereum & \cite{samreen2021smartscan, stephens2021smartpulse,tikhomirov2018smartcheck}\\
        &  Wallet griefing &   & \cite{grech2020madmax} \\
    
    \hline

    Memory refer. distinction 
    & Tainted or shadow memory & Ethereum &  \cite{ashouri2020etherolic}\\
        
    \hline 
    
    \multirow{8}{40mm}{Owner information preservation} 
        & Locked amount & Cardano & \cite{seijas2020efficient,Seijas2020Marlowe} \\ 
        \cline{2-4}
        & Deadlock state, Unprotected suicide &   & \cite{nelaturu2020verified}\\ 
        & Leaking Ether &  & \cite{torres2021confuzzius, huang2021precise} \\
        & Tainted owner variable &  & \cite{brent2020ethainter}\\
        & Unfair payment & Ethereum & \cite{li2020protect} \\ 
        & Unprotected \texttt{selfdestruct} &  & \cite{aidee2021vulnerability, huang2021precise} \\ 
        & Unprotected Ether withdrawal \& vulnerable access control &  & \cite{zhang2020ethploit, stephens2021smartpulse, tsankov2018securify} \\
   
    \hline
          
    Predictable variable usage 
        & Dependence on predictable variables &  Ethereum & \cite{lu2021neucheck, ma2021pluto, nguyen2020sfuzz, wang2020contractward,ashouri2020etherolic, wei2020smart, teng2021SmartGift, Oyente2016, kalra2018zeus, grishchenko2018semantic}\\
    \cline{3-4}
        &  &  EOSIO & \cite{li2022eosioanalyzer, Wasai2022}\\
    
    \hline
    
    \texttt{selfdestruct} accessibility 
        & Accessible \texttt{selfdestruct} &  Ethereum & \cite{brent2020ethainter} \\
        \cline{1-2}
        \texttt{selfdestruct} preservation & Tainted \texttt{selfdestruct} & & \\
        
     \hline
     
    State preservation 
        & Reentrancy & Ethereum &
        \cite{ma2021pluto, wustholz2020harvey, xue2020cross, chinen2020ra, schneidewind2020ethor, arganaraz2020detection, qian2020towards, nelaturu2020verified, ashouri2020etherolic, bang2020verification, li2020protect, semantics2020Jiao, samreen2020reentrancy, ji2021security, lu2021neucheck, britten2021using, wang2020contractward, wei2020smart, teng2021SmartGift, andesta2020testing, stephens2021smartpulse, ribeiro2020formal, Oyente2016,tikhomirov2018smartcheck, mossberg2019manticore, grishchenko2018semantic}\\
        
     \hline
     
    State variables declaration 
        &  Improper state variables declaration & Ethereum & \cite{praitheeshan2021solguard}\\
    
    \hline     
    
    \texttt{staticcall} preservation 
        & Problematic \texttt{staticcall} & Ethereum &  \cite{brent2020ethainter}\\
        
    \hline
    
    Sustainability of gas transfer 
        & Transfer of all the gas & Ethereum & \cite{arganaraz2020detection, tikhomirov2018smartcheck}\\
    
    \hline
      
    Transaction c. effectiveness$^\ast$
        &  DoS due to expensive transactions & Ethereum &  \cite{genet2020termination, chen2020gaschecker, li2022smartfast, SmartMixModel2022}\\
     
    \hline
    
    Transaction o. independence 
        &  Transaction ordering dependency & Ethereum &
        \cite{torres2021confuzzius, ashouri2020etherolic, wang2020contractward, Oyente2016, kalra2018zeus,tsankov2018securify, grishchenko2018semantic}\\
      
    \hline
          
    \multirow{2}{45mm}{Transfer function viability}
        & Missed to implement fallback &  Ethereum & \cite{praitheeshan2021solguard}\\
        &  Use of send instead of transfer & Ethereum & \cite{arganaraz2020detection, tikhomirov2018smartcheck} \\

    \hline 

    Transfer value checking
       & Unchecked send bugs &  Ethereum & \cite{yang2020hybrid, stephens2021smartpulse}\\
     
    \hline 
     
    Withdrawal acceptance$^\ast$ 
        & Locking, locked or freezing Ether & Ethereum &
        \cite{lu2021neucheck, nelaturu2020verified, ashouri2020etherolic, xing2020new, wei2020smart, 10.1145/3412841.3442130, stephens2021smartpulse, tikhomirov2018smartcheck,jiang2018contractfuzzer}\\

  \hline
\end{tabular}
}
 \vspace{-7mm}
\end{table*}

==> BackUP/PreviousStatcProperties.tex <==
%%------------ Static Analysis ------------%%
\begin{table*}
 \vspace{-2mm}
\setlength\abovecaptionskip{-0.1\baselineskip}
\setlength\belowcaptionskip{-0.1\baselineskip}
\caption{Properties of smart contracts addressed in the papers adopting static analysis methods}
\label{tab:SAmethods}
\resizebox{\columnwidth}{!}{
\begin{tabular}{
| l |p{18mm} | p{17mm} |p{19mm} | p{43mm} | p{30mm} | p{15mm} |}
    
    \hline
    Property & 
    Abstract Interpretation &
    Control Flow Analysis &
    Taint Analysis &
    Pattern-based Analysis &
    Symbolic Execution &
    Static Type Checking \\
   
    \hline

    State preservation  
        & \cite{schneidewind2020ethor, tsankov2018securify, smaragdakis2021symbolic}
        & \cite{xue2020cross, brent2018vandal}
        & \cite{feist2019slither, NPChecker2019, li2022smartfast, xue2020cross, ali2021sescon}
        & \cite{li2022smartfast, lu2021neucheck, arganaraz2020detection, tikhomirov2018smartcheck, tsankov2018securify, brent2018vandal, SolChecker2022, ali2021sescon} 
        & \cite{chinen2020ra, smaragdakis2021symbolic, ma2021pluto, Oyente2016, MPro2019}
        &  \cite{das2021resource}\\
    
    \hline

        Owner information preservation  
        & \cite{tsankov2018securify, smaragdakis2021symbolic}
        & \cite{brent2020ethainter}
        & \cite{brent2020ethainter}
        & \cite{tsankov2018securify}
        & \cite{smaragdakis2021symbolic, seijas2020efficient, Seijas2020Marlowe}
        & \cite{zkay1.0, baumann2020zkay} \\
     
    \hline

    
    Integer over/underflow guarding  
        & \cite {Michelson2022}
        & \cite{peng2019sif}
        & \cite{ali2021sescon, Osiris2018, Mythril} 
        & \cite{lai2020static, lu2021neucheck, arganaraz2020detection, tikhomirov2018smartcheck}
        & \cite{permenev2020verx, Osiris2018, Mythril}
        & \\
        
    \hline
        
    Exception \& return value handling  
        & \cite{tsankov2018securify, smaragdakis2021symbolic}
        & \cite{brent2018vandal} 
        & \cite{NPChecker2019, ali2021sescon}
        & \cite{lu2021neucheck, arganaraz2020detection, tikhomirov2018smartcheck, tsankov2018securify, brent2018vandal, SolChecker2022, ali2021sescon}
        & \cite{smaragdakis2021symbolic, ma2021pluto, Oyente2016, Mythril}
        & \\
    
    \hline
    

    \texttt{selfdestruct} accessibility  
        & \cite{smaragdakis2021symbolic}
        & \cite{brent2018vandal}
        & \cite{zhang2020ethploit, ali2021sescon, Mythril}
        & \cite{aidee2021vulnerability, brent2018vandal, ali2021sescon}
        & \cite{smaragdakis2021symbolic, Mythril, MAIAN}
        & \\
        
    \hline

    Transaction order independence 
        & \cite{tsankov2018securify}
        & \cite{tsankov2018securify}
        & \cite{NPChecker2019, ali2021sescon}
        & \cite{tsankov2018securify, ali2021sescon}
        & \cite{Oyente2016}
        & \\
   
    \hline

    Withdrawal acceptance$^\ast$ 
        & \cite{tsankov2018securify}
        & \cite{tsankov2018securify}
        & \cite{li2022smartfast}
        & \cite{li2022smartfast, lu2021neucheck, arganaraz2020detection, tikhomirov2018smartcheck, tsankov2018securify}
        & \cite{MAIAN}
        & \\
        
  \hline
  
    \texttt{delegatecall} preservation  
        & \cite{brent2020ethainter}
        & \cite{brent2020ethainter} 
        & \cite{brent2020ethainter, ali2021sescon}
        & \cite{ali2021sescon}
        & 
        & \\
        
    \hline
    
    
    Boundedness of loops  
        & \cite{grech2020madmax} 
        & \cite{nassirzadeh2021gas}
        &
        & \cite{lu2021neucheck}
        & \cite{seijas2020efficient, Seijas2020Marlowe}
        & \\
    
    \hline
    


    Isolation of external calls  
        & \cite{grech2020madmax} 
        & \cite{grech2020madmax}
        &
        & \cite{tikhomirov2018smartcheck, samreen2021smartscan} 
        & 
        & \\
        
    \hline

    Appropriate address usage  
        &
        & \cite{brent2018vandal}
        & \cite{li2022smartfast}
        & \cite{li2022smartfast, lu2021neucheck, arganaraz2020detection, tikhomirov2018smartcheck, brent2018vandal, zhou2018security}
        & \cite{MAIAN, zhdarkin2021development}
        &  \\
    
    \hline
    
    \texttt{staticcall} info. sustainability  
        & 
        & \cite{brent2020ethainter}
        & \cite{brent2020ethainter, ali2021sescon} 
        & \cite{ali2021sescon} 
        & 
        & \\
    
    \hline

    Information secrecy  
        &
        & \cite{zhang2020ethploit}
        & \cite{zhang2020ethploit}
        & \cite{lu2021neucheck}
        & 
        & \cite{zkay1.0, baumann2020zkay} \\  
    
    \hline

    Divide by zero guarding 
        & 
        & \cite{peng2019sif}
        & 
        & \cite{zhou2018security}
        & \cite{Osiris2018}
        & \\

    \hline
    
    Predictable variable usage 
        &
        &
        & \cite{ali2021sescon, li2022smartfast}
        & \cite{li2022smartfast, li2022eosioanalyzer, lu2021neucheck, arganaraz2020detection, tikhomirov2018smartcheck, zhou2018security, SolChecker2022, ali2021sescon}
        & \cite{yang2020seraph, ma2021pluto, Oyente2016, Mythril}
        & \\
    
    \hline

    Balance comparison  
        &
        &
        & \cite{ali2021sescon}
        & \cite{lu2021neucheck, arganaraz2020detection, tikhomirov2018smartcheck, SolChecker2022, ali2021sescon}
        & 
        & \\
    
    \hline
    
    Argument validation
        & \cite{tsankov2018securify} 
        &
        &
        & \cite{tsankov2018securify} 
        &
        & \\
    \hline   
    
    Eventual contract termination$^\ast$ 
        & \cite {Michelson2022} %theorem prov: \cite{genet2020termination}
        & 
        & 
        & 
        & \cite{seijas2020efficient, Seijas2020Marlowe}
        & \\
    
    \hline
    Deposit validity 
        &
        &
        &
        & \cite{li2022eosioanalyzer} 
        & \cite{he2020security, he2021eosafe, ji2020deposafe}
        & \\
    
    \hline
    
    Address integrity 
    %fuzzer: huang2020eosfuzzer, , Wasai2022
   %modelchecking: nelaturu2020verified
        &
        &
        &  
        & \cite{li2022eosioanalyzer} 
        & \cite{he2021eosafe}
        & \\
    
    \hline
    
    Transfer value checking  
        & 
        & 
        & \cite{zhang2020ethploit}
        & 
        &
        & \\
    
    \hline
    Sustainability of gas transfer 
        &
        &
        & 
        & \cite{arganaraz2020detection, tikhomirov2018smartcheck, aidee2021vulnerability}
        & 
        & \\
    
    \hline
    
    Transfer function viability  
        &
        &
        & 
        & \cite{praitheeshan2021solguard, arganaraz2020detection, tikhomirov2018smartcheck}
        &
        & \\
    \hline

   
    
    State variable... \& Address parameter...
        &
        &
        &
        & \cite{praitheeshan2021solguard} 
        &
        & \\
    
    \hline
    
    Explicit access control modifier usage 
        &
        &  
        &
        & \cite{lu2021neucheck, tikhomirov2018smartcheck} 
        &
        & \\
    
    \hline
    
    Eventual termination of expressions$^\ast$...
        &
        &
        &
        & \cite{lu2021neucheck, arganaraz2020detection} 
        &
        & \\
    
    \hline
    
    Floating point guarding
        &
        &
        &
        & \cite{arganaraz2020detection, tikhomirov2018smartcheck} 
        &
        & \\
    \hline    

    Hash collision freeness  
        &
        &
        & 
        & \cite{lu2021neucheck}
        &
        & \\
    
    \hline
    
    Asset preservation  
        &
        &
        &
        &
        &
        & \cite{10.1007/978-3-030-54455-3_41, das2021resource, coblenz2020obsidian} \\

  

        \hline

\end{tabular}
}
\vspace{-6mm}
\end{table*}


==> BackUP/T_MachineLearning.tex <==
%%------------ Table for Properties in ML methods ------------%%

\begin{table*}
 \vspace{-2mm}
\setlength\abovecaptionskip{-0.1\baselineskip}
\setlength\belowcaptionskip{-0.1\baselineskip}
\caption{Properties of smart contracts addressed in the papers adopting machine learning methods}
\label{tab:MLmethods}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|l |c | c |c |c | c | c | c |c |}
    \hline
    Property & Supervised Classification & NLP & ANN & GNN & CNN & RNN  & DNN & LSTM\\
    
    \hline
    State preservation
        & \cite{wang2020contractward, xu2021novel}
        & \cite{ashizawa2021eth2vec}
        &
        & \cite{zhuang2020smart, liu2021combining}
        &
        & \cite{qian2020towards}
        & \cite{mi2021vscl, SVChecker2022} 
        & \cite{HAMBiLSTM2022}\\
     \hline
     
    Integer over/underflow guarding
        & \cite{wang2020contractward, xu2021novel}
        & \cite{ashizawa2021eth2vec}
        &
        &
        & \cite{xing2020new}
        &
        & \cite{SVChecker2022}
        & \\
     \hline
    Values unpredictability
        & \cite{wang2020contractward, xu2021novel}
        & \cite{ashizawa2021eth2vec}
        &
        & \cite{zhuang2020smart, liu2021combining}
        &
        &
        & 
        & \\
     \hline

    Transaction order... \& Exception. handling
        & \cite{wang2020contractward, xu2021novel}
        &
        &
        &
        &
        &
        & \cite{SVChecker2022}
        & \\
    \hline
    Transaction cost boundedness
        &
        & 
        &
        &
        &
        &
        & \cite{SmartMixModel2022}
        & \\
         \hline
    Deposit Validity \& Explicit access control... 
        &
        & \cite{ashizawa2021eth2vec}
        &
        &
        &
        &
        & 
        & \\
    \hline

    Appropriate address usage
        &
        &
        & \cite{GUPTA2021107583, narayana2021automation}
        &
        &
        &
        & \cite{SmartMixModel2022}
        & \\
         \hline
    Transfer function viability
        & \cite{hao2020scscan}
        &
        & \cite{GUPTA2021107583, narayana2021automation}
        &
        &
        &
        &
        & \\
         \hline

    Boundedness of loops
        & \cite{xu2021novel, narayana2021automation}
        &
        &
        & \cite{zhuang2020smart, liu2021combining}
        &
        &
        & 
        & \\
     \hline
    Address size soundness
        & 
        &
        &
        &
        & \cite{xing2020new}
        &
        & 
        & \\
         \hline
    Withdrawal acceptance$^\ast$ \& Balance comp...
        &
        &
        &
        &
        &
        &
        & \cite{SmartMixModel2022}
        & \\
        
    \hline

\end{tabular}
}
\vspace{-6mm}
\end{table*}

==> T10_NumberOfPropMethods.tex <==
%%------------ Table for # of Properties & methods per platform------------%%
\begin{table*}
  \caption{Number of properties (Section \ref{properties}) \& analysis methods (Section \ref{methods}) for individual platforms}
  \label{tab:propsmethods}
 %  \vspace{-4mm}
      \resizebox{\columnwidth}{17mm}{
  \begin{tabular}{| l |c | c | p{125mm} |}
    \hline
    Platform & 
    \# of properties &
    \# of Analyses &
    Study\\
    \hline
    Ethereum & 22 & 73 & \cite{li2020protect, wustholz2020harvey, ashouri2020etherolic, sun2020formal, permenev2020verx, hajdu2019solc, so2020verismart, bang2020verification, albert2020taming, schneidewind2020ethor, zhang2020smartshield, zhang2020ethploit, brent2020ethainter, xue2020cross, antonino2020formalising, lai2020static, nelaturu2020verified, baumann2020zkay, grieco2020echidna, arganaraz2020detection, grech2020madmax, lu2021neucheck, schiffl2021towards, ma2021pluto, bram2021rich, Correas2021static, britten2021using, osterland2020model, wesley2021compositional, duo2020formal, marescotti2020accurate, gao2021sverify, stephens2021smartpulse, ahrendt2020functional, elad2021summing, mazurek2021ethver, samreen2020reentrancy, ivanova2020regularmutator, andesta2020testing, huang2021precise,ji2020deposafe,aidee2021vulnerability, yang2020hybrid, chinen2020ra, yang2020seraph, chen2020gaschecker, smaragdakis2021symbolic, zhdarkin2021development, wang2021mar,wang2020oracle, soto2020fuzzing, nguyen2020sfuzz, wei2020smart, teng2021SmartGift, mi2021vscl, narayana2021automation, GUPTA2021107583, xu2021novel, qian2020towards, hao2020scscan,  wang2020contractward, xing2020new, zhuang2020smart,ashizawa2021eth2vec, huang2021hunting,liu2021combining, chen2021one, torres2021confuzzius, albert2021don, albert2020analyzing, ali2021sescon,contro2021ethersolve, das2021resource}\\
    
    \hline
    Tezos & ? & 12 & \cite{da2020whylson, nishida2022helmholtz, 10.1007/978-3-030-54455-3_41, 10.1007/978-3-030-61467-6_5, perez2020cost, 9284726, goes2020compiling, reis2020tezla, Mi-Cho-Coq2020, annenkov2021extracting,milo2022finding, Michelson2022}\\
    \hline
    Libra Blockchain & 2 & 4 & \cite{zhong2020move, patrignani2021robust, das2020exact, blackshear2020resources} \\
    \hline
    EOSIO & 3 & 5 & \cite{huang2020eosfuzzer, he2021eosafe, li2022eosioanalyzer,Wasai2022, he2020security}\\
    \hline
    HyperLedger Fabric & ? & 4 & \cite{coblenz2020obsidian, ding2021hfcontractfuzzer,jiang2018contractfuzzer, 8859497} \\
    \hline
    Algorand & 1 & 1 & \cite{bartoletti2021formal} \\
     \hline 
     Zilliqa & ? & 3 & \cite{sergey2018temporal, Scilla2018, Scilla2019} \\
    \hline 
     Cardano & 3 & 2 & \cite{seijas2020efficient, Seijas2020Marlowe} \\
      \hline 
     Azure & ? & 2 & \cite{verification2018Azure, wang2019formal} \\
    \hline
  %  Bitcoin & 1 & 2 & \cite{atzei2019developing, simplicity2017Russel}\\
    
   \hline
\end{tabular}
}
 %  \vspace{-4mm}
\end{table*}

==> T3_ComparisonRelatedSurveys.tex <==
 %%------------ Table of comparison with related surveys  ------------%%
\begin{table*}
% \vspace{-2mm}
\small
\setlength\abovecaptionskip{-0.1\baselineskip}
\begin{minipage}{\columnwidth}   
  \caption{Number of vulnerabilities and tools reviewed and categorization type adopted in related surveys}
  \label{tab:comparison2}
    %  \vspace{-4mm}
    \resizebox{\columnwidth}{!}{
  \begin{tabular}{|l | c | p{20mm} | p{80mm} |}
    \hline
    \textbf{Survey} & \textbf{Vulnerabilities} & 
    \textbf{Analysis Tools}
    &  \textbf{Categorization Type of Vulnerabilities}\\
    \hline
    This Survey
    & 55 & 78 (review) & 
    Violations to properties \\
       \hline
   H. Chen et al., 2020 \cite{chen2020survey} & 
   44 (21 common) & 24 (review)\footnote{The survey \cite{chen2020survey} reviews forty-seven defenses, out of which twenty-four are analysis tools.}&
   \romannumeral 1) root cause, 
    \romannumeral 2) occurrences layer,
    \romannumeral 3) status \\
     \hline
    Gupta et al.,2020 \cite{gupta2020insecurity} & 
    38(26 common) & 6 (evaluation)& 
    Hierarchical categorization w.r.t source and type\\
         \hline
   Demir et al., 2019 \cite{demir2019security} & 
     28 (18 common) & 
   4 (review)  &
   \romannumeral 1) dependence on the environment, 
 \romannumeral 2) design and deployment issues, 
 \romannumeral 3) misuse of trust,
 \romannumeral 4) control of execution, 
 \romannumeral 5) reentrancy, unsafe external interaction, and vulnerable coding practices \\
     \hline
  Staderini et al., 2020  \cite{staderini2020classification} & 
     28 (23 common)
    & 0 &
    CWE-classes~\footnote{A community-developed list of software and hardware weekness types, \url{https://cwe.mitre.org/data/index.html}} (10)\\
     \hline
  Dika \& Nowostawski, 2018 \cite{dika2018security} & 
    22 (16 common) & 4 (evaluation) & 
    \romannumeral 1) architectural level
\romannumeral 2)  severity (1 to 3)
\\
     \hline
  Mense \& Flatscher, 2018 \cite{menseVulnerabilities} & 
   22 (16 common) &  7 (evaluation) & 
    \romannumeral 1) architectural level
\romannumeral 2)  severity (1 to 3)
\\
     \hline
   Groce et al., 2020 \cite{groce2020actual} &
    22 (10 common)
    & 0 & 
    Severity \& difficulty \\
     \hline
   Chen et al., 2020 \cite{chen2020Defects} &
    20(10 common)
    & 0 &
    \romannumeral  1) security, 
    \romannumeral  2) availability,
    \romannumeral  3) performance
    \romannumeral  4) maintainability,
    \romannumeral  5) reusability \\
       \hline  
  Khan \& Namin, 2020 \cite{khan2020survey} &
    16 (all common) & 24 (review) &
    \romannumeral  1) inter-contractual/contractual vulnerabilities, 
    \romannumeral  2) arithmetic bugs, 
    \romannumeral  3) gas-related issues,
    \romannumeral  4) transactional irregularities \\
     \hline
  Yamashita et al., 2019 \cite{yamashitaPotentialRisks} &
   16 (2 common) &  1 (evaluation) &
    Potential risks: non-determinism, state database specification, fabric specification, and common practices \\
     \hline
   Atzei et al., 2017 \cite{atzei2017survey} & 
     12(8 common)
    & 0 &
    Sources (Solidity, EVM bytecode, \& blockchain) \\
     \hline
  Liehuang et al., 2018  \cite{zhu2018research} &
     11(5 common)
    & 0 &
    \romannumeral 1) logic problems,
    \romannumeral 2) semantic misunderstanding,
    \romannumeral 3) design problems,
    \romannumeral 4) privacy-preserving \\
     \hline
   Z. Li et al., 2020 \cite{li2020research} &
    7 (4 common)
    & 0 & 
    Layers (Blockchain, contract) \\
     \hline
   He, Daojing et al. 2020 \cite{He9143290}&
   10 (9 common) & 3 (evaluation)
     & No classification\\
     \hline
   Krupa et al., 2020 \cite{krupa2021security}&
    10 (8 common) &  2 (review)
     & No classification\\
     \hline
 Rahimian \& Clark, 2021 \cite{rahimian2021tokenhook}& 
       9 (8 common) &  7 (evaluation)
        & No classification\\
        \hline
   Ji, Suhwan et al., 2021 \cite{ji2021evaluating} &
     9 (all common) &  1 (evaluation)
 & No classification\\
 \hline
\end{tabular}
}
\end{minipage}
\setlength\belowcaptionskip{-0.1\baselineskip}
 %    \vspace{-6mm}
\end{table*}

==> T4_PropertiesVulnerabilities.tex <==
%%------------ Table of Properties vs vulnerabilities ------------%%
\begin{table*}
% \vspace{-2mm}
\small
\setlength\abovecaptionskip{-0.1\baselineskip}
 \setlength\belowcaptionskip{-0.2\baselineskip}
  \caption{Smart contract properties with related vulnerabilities and studies}
  \label{tab:propVuln}
   \resizebox{\columnwidth}{100mm}{
  \begin{tabular}{| p{40mm} | p{46mm} | p{12mm} | p {60mm} |}
    \hline
    Property & Vulnerabilities & Platform & Studies \\
    \hline

    \multicolumn{4}{| l | }{\textbf{Liveness}} \\
    \hline
 
    Deposit acceptance 
        &  Failing to accept new deposit & Ethereum & \cite{park2020end} \\
    \hline

    Eventual contract removal & References to destroyed contracts & Ethereum & \cite{nelaturu2020verified}\\
       \hline
    %\multirow{2}{45mm}{
    Eventual contract termination %} 
        & Non-terminating contracts 
        %& Ethereum & \cite{genet2020termination}  \\
        %&  \cline{3-4}
        %&   
        & Cardano & \cite{seijas2020efficient,Seijas2020Marlowe} \\
    \hline
    
    Withdrawal acceptance 
        & Locking, locked or freezing Ether & Ethereum &
        \cite{lu2021neucheck, nelaturu2020verified, ashouri2020etherolic, xing2020new, wei2020smart, 10.1145/3412841.3442130, stephens2021smartpulse, tikhomirov2018smartcheck,jiang2018contractfuzzer}\\

    \hline
    \addlinespace[1mm] 
    \hline

    \multicolumn{4}{| l | }{\textbf{Safety}} \\
    \hline
    
    \multirow{2}{45mm}{Address integrity}
        & Forged notification, Fake receipt & EOSIO & \cite{huang2020eosfuzzer, he2021eosafe, li2022eosioanalyzer,Wasai2022} \\
        \cline{2-4}
        & External contract referencing & Ethereum & \cite{nelaturu2020verified} \\
    \hline
    
    Address parameter avoidance 
        & Misuse of address parameters  & Ethereum & \cite{praitheeshan2021solguard}\\
        
    \hline
    Address size soundness 
        & Address shortening & Ethereum & \cite{nelaturu2020verified, ashouri2020etherolic, xing2020new}\\
           
    \hline
           
    \multirow{2}{45mm}{Appropriate address usage}
        & Misuse of \texttt{msg.sender} &   & \cite{zhdarkin2021development}\\
        & Misuse of \texttt{tx.origin}  & Ethereum &  \cite{lu2021neucheck, arganaraz2020detection, kalra2018zeus, tikhomirov2018smartcheck, brent2018vandal}\\
        & Prodigal contract & & \cite{praitheeshan2019security, tang2021vulnerabilities}\\
        
    \hline

    Argument precond. validation & Use of untrusted arguments & Ethereum & \cite{tsankov2018securify} \\
    \hline
    
    Balance comparison 
        & Strict equality of balance &  Ethereum & \cite{lu2021neucheck, arganaraz2020detection,tikhomirov2018smartcheck} \\
    
    \hline
           
    \multirow{3}{45mm}{Boundedness of loops}    
        & Un-bounded mass operations & Ethereum &  \cite{grech2020madmax, lu2021neucheck, nassirzadeh2021gas, Correas2021static}\\
        & Unsafe type declaration &  & \cite{lu2021neucheck, arganaraz2020detection, tikhomirov2018smartcheck} \\
      \hline
      
       Conditional independence  
        & DoS due to external contracts & Ethereum & \cite{arganaraz2020detection, lu2021neucheck}\\
    \hline
        

    
    Division by zero guarding 
        & Unchecked division by zero & Ethereum & \cite{so2020verismart, Khor2020improved, Osiris2018}\\
    
    \hline
    
    Effective callback freeness & Reentrancy & Ethereum
        &\cite{albert2020taming, grossman2017online}\\   
    
    \hline
    
    \multirow{3}{40mm}{Exception \& return value handling}   
        & Callstack depth issue &   & \cite{wang2020contractward}\\
        & Gasless send &  Ethereum & \cite{nguyen2020sfuzz, teng2021SmartGift, jiang2018contractfuzzer} \\
        & Mishandled/unhandled exceptions &  & \cite{zhang2020smartshield, nelaturu2020verified, ashouri2020etherolic, arganaraz2020detection, semantics2020Jiao, nguyen2020sfuzz, wei2020smart, Oyente2016, kalra2018zeus, tikhomirov2018smartcheck, grishchenko2018semantic}\\ 
    
    \hline
    
    \multirow{2}{40mm}{Explicit access control modifiers usage}
        & Tainted owner, Vulnerable access & Ethereum & \cite{lu2021neucheck} \\
        & Unspecified visibility level &  &  \cite{lu2021neucheck, tikhomirov2018smartcheck} \\
    
    \hline

    Gas transfer viability 
        & Transfer of all the gas & Ethereum & \cite{arganaraz2020detection, tikhomirov2018smartcheck}\\
    
    \hline
    
    Guarding of \texttt{selfdestruct} 
        & Accessible \texttt{selfdestruct} &  Ethereum & \cite{brent2020ethainter} \\
        \cline{1-2}
        Preservation of \texttt{selfdestruct} & Tainted \texttt{selfdestruct} & & \\
        
     \hline
     
     Information secrecy 
        &  Exposed secret & Ethereum & \cite{zhang2020ethploit, lu2021neucheck}\\
    
    \hline 
    
    Integer division guarding 
        & Unexpected results from divisions 
        & Ethereum 
        & \cite{arganaraz2020detection, tikhomirov2018smartcheck}\\
    \hline
    
    Integer over/underflow guarding 
        &  Integer over/underflow  & Ethereum 
        & \cite{ma2021pluto, ashouri2020etherolic, sun2020formal, so2020verismart, lai2020static, xing2020new, semantics2020Jiao, nguyen2020sfuzz, Khor2020improved, wang2020contractward, lu2021neucheck, yang2020hybrid, andesta2020testing,stephens2021smartpulse, kalra2018zeus,mossberg2019manticore} \\
        \cline{3-4}
        &  & H. Fabric & \cite{ding2021hfcontractfuzzer}\\
    
    \hline
    
    \multirow{2}{45mm}{Isolation of external calls}
        & DoS due to external contracts & Ethereum & \cite{samreen2021smartscan, stephens2021smartpulse,tikhomirov2018smartcheck}\\
        &  Wallet griefing (\ref{P_isolationofcalls}) &   & \cite{grech2020madmax} \\
    
    \hline
    
    Map disjointness 
        & Map overlap &  Ethereum & \cite{lu2021neucheck}\\
    
    \hline
    
    Memory refer. distinction 
    & Tainted or shadow memory & Ethereum &  \cite{ashouri2020etherolic}\\
    \hline 
    
    Ownership of assets 
        & Improper handling of assets 
        & Ethereum & \cite{bram2021rich} \\
    
    \hline
    
    Preservation of assets & Improper handling of assets & Libra & \cite{blackshear2020resources}\\
    \cline{3-4}
    & & H. Fabric & \cite{coblenz2020obsidian}\\
    \cline{3-4}
    & & Ethereum &\cite{bram2021rich} \\
    \hline

    \multirow{2}{45mm}{Preservation of assets in transactions}
        & Unfair payment & Ethereum &\cite{li2020protect} \\ 
        \cline{2-4}
        &  Double-spending  & Algorand &\cite{bartoletti2021formal}\\
          
    \hline
    
    Guarding of \texttt{delegatecall} 
        & Tainted/dangerous \texttt{delegatecall} & Ethereum & \cite{brent2020ethainter, wei2020smart, teng2021SmartGift, andesta2020testing, jiang2018contractfuzzer} \\
         
    \hline
    
    Preservation of \texttt{staticcall} 
        & Problematic \texttt{staticcall} & Ethereum &  \cite{brent2020ethainter}\\
        
    \hline
    
     \multirow{8}{40mm}{Preservation of owner information} 
        & Locked amount & Cardano & \cite{seijas2020efficient,Seijas2020Marlowe} \\ 
        \cline{2-4}
        & Deadlock state, Unprotected suicide &   & \cite{nelaturu2020verified}\\ 
        & Leaking Ether &  & \cite{torres2021confuzzius, huang2021precise} \\
        & Tainted owner variable &  & \cite{brent2020ethainter}\\
        & Unfair payment & Ethereum & \cite{li2020protect} \\ 
        & Unprotected \texttt{selfdestruct} &  & \cite{aidee2021vulnerability, huang2021precise} \\ 
        & Unprotected withdrawal &  & \cite{zhang2020ethploit, stephens2021smartpulse, tsankov2018securify} \\
   
    \hline 
    
    Preservation of state 
        & Reentrancy & Ethereum &
        \cite{ma2021pluto, wustholz2020harvey, xue2020cross, chinen2020ra, schneidewind2020ethor, arganaraz2020detection, qian2020towards, nelaturu2020verified, ashouri2020etherolic, bang2020verification, li2020protect, semantics2020Jiao, samreen2020reentrancy, ji2021security, lu2021neucheck, britten2021using, wang2020contractward, wei2020smart, teng2021SmartGift, andesta2020testing, stephens2021smartpulse, ribeiro2020formal, Oyente2016,tikhomirov2018smartcheck, mossberg2019manticore, grishchenko2018semantic}\\
        
     \hline
     
    State variables declaration ord.
        &  Improper state variables declaration & Ethereum & \cite{praitheeshan2021solguard}\\
    
    \hline  
    
    Transaction cost boundedness
        &  DoS due to expensive transactions & Ethereum &  \cite{genet2020termination, chen2020gaschecker, li2022smartfast, SmartMixModel2022}\\
    \hline
    
    Transaction o. independence 
        &  Transaction ordering dependency & Ethereum &
        \cite{torres2021confuzzius, ashouri2020etherolic, wang2020contractward, Oyente2016, kalra2018zeus,tsankov2018securify, grishchenko2018semantic}\\
      
    \hline

    Transfer amount boundedness  
        & Unrestricted amount transfer & Cardano
        & \cite{seijas2020efficient, Seijas2020Marlowe} \\
    \hline
    
    \multirow{2}{45mm}{Transfer function viability}
        & Missed to implement fallback &  Ethereum & \cite{praitheeshan2021solguard}\\
        &  Use of send instead of transfer &  & \cite{arganaraz2020detection, tikhomirov2018smartcheck} \\

    \hline 
    
    \multirow{2}{45mm}{Validity of deposits}
        & Fake deposit & Ethereum & \cite{ji2020deposafe} \\
        \cline{2-4}
        & Fake EOS & EOSIO & \cite{he2020security, huang2020eosfuzzer, he2021eosafe, li2022eosioanalyzer, Wasai2022} \\
        \cline{2-4}
        & Negative deposit & Cardano &  \cite{seijas2020efficient}\\
       
    \hline 
    Validity of transfer amount
       & Unchecked send bugs &  Ethereum & \cite{yang2020hybrid, stephens2021smartpulse}\\
     
    \hline 
    
    Value unpredictability 
        & Dependence on predictable variables &  Ethereum & \cite{lu2021neucheck, ma2021pluto, nguyen2020sfuzz, wang2020contractward,ashouri2020etherolic, wei2020smart, teng2021SmartGift, Oyente2016, kalra2018zeus, grishchenko2018semantic}\\
    \cline{3-4}
        &  &  EOSIO & \cite{li2022eosioanalyzer, Wasai2022}\\
    \hline
    
\end{tabular}
}
% \vspace{-7mm}
\end{table*}

==> T9_FrequentProperties.tex <==
%%------------ Table for Frequent Properties ------------%%
\begin{table*}[h]
% \vspace{-2mm}
\setlength\abovecaptionskip{-0.1\baselineskip}
\setlength\belowcaptionskip{-0.1\baselineskip}
  \caption{Five most frequently addressed smart contract properties (Section \ref{properties})}
  \label{tab:commonProperties}

  \resizebox{\columnwidth}{!}{
  \begin{tabular}{| l |p{12mm} | p{95mm} |}
    \hline
    Property & 
    \# of Analyses &
    Study\\
    \hline
    Preservation of state & 26  & \cite{ma2021pluto, wustholz2020harvey, xue2020cross, chinen2020ra, schneidewind2020ethor, arganaraz2020detection, qian2020towards, nelaturu2020verified, ashouri2020etherolic, bang2020verification, li2020protect, semantics2020Jiao, samreen2020reentrancy, ji2021security, lu2021neucheck, britten2021using, wang2020contractward, wei2020smart, teng2021SmartGift, andesta2020testing, stephens2021smartpulse, ribeiro2020formal, Oyente2016,tikhomirov2018smartcheck, mossberg2019manticore, grishchenko2018semantic}\\
    \hline
    Integer over/underflow guarding & 17 & \cite{ma2021pluto, ashouri2020etherolic, sun2020formal, so2020verismart, lai2020static, xing2020new, semantics2020Jiao, nguyen2020sfuzz, Khor2020improved, wang2020contractward, lu2021neucheck, yang2020hybrid, ding2021hfcontractfuzzer, andesta2020testing,stephens2021smartpulse, kalra2018zeus,mossberg2019manticore}\\
    \hline
    Exceptions \& return values handling & 14 & \cite{zhang2020smartshield, nelaturu2020verified, ashouri2020etherolic, arganaraz2020detection, semantics2020Jiao, nguyen2020sfuzz, wei2020smart, Oyente2016, kalra2018zeus, tikhomirov2018smartcheck, grishchenko2018semantic, wang2020contractward, teng2021SmartGift, jiang2018contractfuzzer} \\
    \hline
Owner information preservation & 12 & \cite{seijas2020efficient, Seijas2020Marlowe, brent2020ethainter, li2020protect, torres2021confuzzius, huang2021precise, zhang2020ethploit, stephens2021smartpulse, tsankov2018securify, aidee2021vulnerability, kalra2018zeus, nelaturu2020verified}\\
    
   \hline
    Gas-related properties & 10 & \cite{Correas2021static, arganaraz2020detection, reis2020tezla, nguyen2020sfuzz, albert2021don, grech2020madmax, lu2021neucheck, nassirzadeh2021gas, tikhomirov2018smartcheck, aidee2021vulnerability} \\
     \hline
    
\end{tabular}
}
 %  \vspace{-4mm}
\end{table*}

==> T9_PropertiesFormalization.tex <==
%%------------ Table for formalization of Properties ------------%%
\begin{wraptable}{r}{6.5cm}
\tiny
\setlength\abovecaptionskip{-0.1\baselineskip}
 \setlength\belowcaptionskip{-0.2\baselineskip}
  \caption{Formalization of properties}
  \label{tab:formalProperties}
  \begin{tabular}{| l |p{22mm}|}
    \hline
    Property & 
    Formalized in the studies \\
    \hline
    Address size soundness \& Eventual contract removal &  \cite{nelaturu2020verified}\\
    \hline
    Guarding of delegatecall  & \cite{semantics2020Jiao}\\
    \hline
    Eventual contract termination & \cite{genet2020termination} \\
    \hline
    Isolation of external calls  & \cite{stephens2021smartpulse}\\
   \hline
    Preservation of assets in transactions  & \cite{bartoletti2021formal} \\
     \hline
     Guarding of selfdestruct  & \cite{kalra2018zeus,nelaturu2020verified}\\
     \hline
     Validity of transfer amount  & \cite{stephens2021smartpulse,yang2020hybrid}\\
         \hline
     Withdrawal acceptance & \cite{nelaturu2020verified,stephens2021smartpulse}\\
         \hline
     Transaction order independence & \cite{grishchenko2018semantic,kalra2018zeus}
     %duo2020formal
     \\
         \hline
     Validity of transfer address & \cite{kalra2018zeus,ATL2022,nguyen2021sguard} \\
         \hline
     Exception return value handling  & \cite{grishchenko2018semantic, semantics2020Jiao,kalra2018zeus,nelaturu2020verified} \\
         \hline
     Functional annotations and assertions & \cite{marescotti2020accurate} %SolCMC2022,duo2020formal
     \\
         \hline
     Value unpredictability  & \cite{ grishchenko2018ethertrust,grishchenko2018foundations, grishchenko2018semantic,kalra2018zeus} 
     %duo2020formal
     \\
         \hline
     Integer over/underflow guarding  & \cite{semantics2020Jiao, kalra2018zeus,nguyen2021sguard,stephens2021smartpulse,yang2020hybrid} %SolCMC2022
     \\
         \hline
     Preservation of state & \cite{britten2021using,grishchenko2018ethertrust,grishchenko2018foundations, grishchenko2018semantic,semantics2020Jiao,kalra2018zeus, Mavridou2018, verisolid2019, ATL2022,nelaturu2020verified,nguyen2021sguard,stephens2021smartpulse}%ahrendt2020functional,SPARK2019,SolCMC2022,duo2020formal
     %
     \\
         \hline
\end{tabular}
%}
\end{wraptable}

==> T_StudiesPerMethod.tex <==
\begin{comment}
\begin{table*}
\setlength\abovecaptionskip{-0.1\baselineskip}
  \setlength\belowcaptionskip{-0.1\baselineskip}
  \caption{Analysis methods (Section \ref{methods}) adopted by tools and approaches}
  \label{tab:analysismethods}
  %  \vspace{-4mm}
    \resizebox{\columnwidth}{15mm}{
  \begin{tabular}{| l |c | p{150mm} |}
    \hline
    Analysis Method & 
    \# of Tools &
    Study\\
    \hline
    Static Analysis & 28  & \cite{schneidewind2020ethor, grech2020madmax, brent2020ethainter, zhang2020ethploit, xue2020cross, arganaraz2020detection, lai2020static, aidee2021vulnerability, ali2021sescon, praitheeshan2021solguard, lu2021neucheck, samreen2021smartscan, albert2020taming, albert2021don, Correas2021static, nelaturu2021smart, perez2020cost, lagouvardos2020precise, albert2020analyzing, contro2021ethersolve,baumann2020zkay,nishida2022helmholtz,das2021resource,safe2020rezaei,yang2020lolisa,hamdaqa2020icontractml,mariano2020demystifying,coblenz2020obsidian}\\
    
    \hline
    Formal Verification & 38 & \cite{sun2020formal, da2020whylson,Mi-Cho-Coq2020, yang2020hybrid, nelaturu2020verified,bang2020verification, antonino2020formalising, osterland2020model, wesley2021compositional, duo2020formal, hajdu2019solc, marescotti2020accurate, so2020verismart, gao2021sverify, permenev2020verx, chinen2020ra, yang2020seraph, chen2020gaschecker, he2020security, he2021eosafe, ma2021pluto, smaragdakis2021symbolic, zhdarkin2021development, zhong2020move, patrignani2021robust, stephens2021smartpulse, das2020exact, ahrendt2020functional, han2020formal, hajdu2020formal, ribeiro2020formal, jiao2020generalized, bram2021rich, arusoaie2021certifying, annenkov2020concert,milo2022finding, annenkov2021extracting, mazurek2021ethver, britten2021using, elad2021summing, bartoletti2021formal}\\
    \hline
    Dynamic Analysis & 16 & \cite{li2020protect, huang2021precise,wang2021mar,wustholz2020harvey,grieco2020echidna,wang2020oracle,soto2020fuzzing,nguyen2020sfuzz,wei2020smart,huang2020eosfuzzer,ding2021hfcontractfuzzer,torres2021confuzzius,andesta2020testing,ivanova2020regularmutator,teng2021SmartGift,chen2021one} \\
    \hline
    Machine Learning & 12 & \cite{qian2020towards, hao2020scscan,wang2020contractward, xing2020new,zhuang2020smart,ashizawa2021eth2vec,huang2021hunting,liu2021combining,xu2021novel,GUPTA2021107583,narayana2021automation,mi2021vscl} \\
    
   \hline
\end{tabular}
}
\end{table*}
\end{comment}
